Think Like Human Developers: Harnessing Community Knowledge for Structured Code Reasoning

Large Language Models (LLMs) have significantly advanced automated code generation, yet they struggle with complex coding tasks requiring multi-step logical reasoning. High-quality reasoning data is crucial for improving LLMs' reasoning capabilities, but such datasets remain scarce. Existing approaches either rely on computationally expensive reinforcement learning (RL) or error-prone reasoning chains synthesized by LLMs, posing challenges in scalability and accuracy. To address this challenge, we propose SVRC (Structured and Validated Reasoning Chains for Code Generation), a novel framework that mines, restructures, and enriches reasoning chains from community-driven discussions on software engineering platforms. SVRC refines unstructured and incomplete discussions of coding problems by aligning them with Software Development Life Cycle (SDLC) principles, ensuring that reasoning chains capture real-world problem-solving strategies and support iterative refinement. To evaluate the effectiveness of SVRC, we introduce CodeThinker, an LLM fine-tuned on 12,444 reasoning-augmented samples generated by SVRC. Experiments on LiveCodeBench show that CodeThinker surpasses its base model by 42.86\% on medium-level code problems in terms of pass@1 and outperforms GPT-4o-mini and GPT-4o by 73.14\% and 115.86\%, respectively. Our ablation study further highlights that each component of SVRC contributes to the reasoning capabilities of CodeThinker.

==> dataset.tex <==
\subsection{Dataset Generation}

We generate a dataset for reasoning from two resources.

\textbf{LeetCode} One is from Leetcode, which we collect the gt solutions from community and re-write them to simulate the reasoning process of human solving the coding tasks.

\textbf{APPS} We also apply rejection sampling to generate reasoning steps from existing datsaet. The rejection criteria is whether the LLM can generate the code that passes the test cases given the task and the reasoning steps.

\subsubsection{Reasoning Steps Definition}
Can summarize from QWQ-32B but reference required. 
Refer to software development life cycle.
\begin{itemize}
    \item Requirements gathering and analysis: When faced with a coding task, the first step is to understand the problem thoroughly. This involves reading the problem statement carefully and ensuring all requirements and constraints are clear. 
    \item Planning: Once the problem is understood, the next step is to think about possible approaches to solve it. This often involves breaking down the problem into smaller, more manageable subproblems. For example, if the task is to sort a list of numbers, one might consider different sorting algorithms like bubble sort, quicksort, or mergesort, and evaluate which one would be most efficient given the constraints.
    \item Design: After selecting an approach, it's helpful to sketch out a plan or outline of the steps needed to implement the solution. This can be done mentally or by jotting down notes. For instance, if choosing to implement quicksort, one would need to define the partitioning logic, the recursive sorting of subarrays, and the base case for recursion.
    \item Development: Once the plan is in place, the next step is to start coding. It's important to write clean, readable code that is well-commented, especially if the algorithm is complex. Following best practices in coding, such as using meaningful variable names and maintaining consistent indentation, can make the code easier to understand and debug.
    \item Optimizing in Circle: During the coding phase, it's common to encounter obstacles or realize that the initial approach isn't working as expected. In such cases, it's necessary to revisit the plan and make adjustments as needed. This might involve tweaking the algorithm, refactoring the code, or trying a completely different approach.

Testing is a crucial part of the coding process. It's important to write test cases that cover various scenarios, including edge cases and potential error-prone situations. For example, when testing a sorting algorithm, one should test with an empty list, a list with one element, a list with duplicate elements, and lists that are already sorted or sorted in reverse order.

After implementing the solution and testing it, it's beneficial to review the code and see if any optimizations can be made. This could involve reducing the time complexity, minimizing memory usage, or simplifying the code for better readability.

Finally, once the code is working correctly and is optimized as much as possible, it's time to submit the solution or integrate it into the larger system, depending on the context.
\end{itemize}

\subsection{Leetcode Dataset Generation}

\subsubsection{Explore the potential of existing LLM to generate reasoning steps}

Given the original question, gt code, and raw reasoning steps, ask the LLM to generate the reasoning steps that reflect the above definition.

\textbf{QWQ-32B}
\textbf{delete }We collected the data, to ensure the different token usage for diverse difficulty level, we set some empirical numbers. 

Statistic on easy question:
count     4043.000000 \\
mean      3212.188721 \\
std       1835.739043\\
min        300.000000\\
25\%       2138.500000\\
50\%       2814.000000\\
75\%       3848.000000\\
max      16000.000000\\
Therefore we set the valid data as token numbers between 2000 to 5000, ending with 2710 reasoning data. 

Statistic on medium question:
count     9813.000000
mean      5397.022419
std       2867.023231
min        332.000000
25%       3532.000000
50%       4854.000000
75%       6773.000000
max      16000.000000 \\
Therefore we set the valid data as token numbers between 2500 to 8000, ending with 7154 reasoning data. 

Statistic on hard question:
count     3527.000000
mean      6608.124185
std       3517.316538
min        475.000000
25%       4247.500000
50%       6401.000000
75%       8877.000000
max      16000.000000 \\
Therefore we set the valid data as token numbers between 3500 to 12000, ending with 2610 reasoning data. 

In total 12474 obtained

I also filtered out around 300 answers that code blocks have more than 1. finally 12244.

\subsubsection{Experiment Result}
We apply the 12474 data to fine-tune DeepseekCoder 32B for one epoch. 

The result is shown as below: the pass@1 is 0.17, lower than the original LLM.

However, after manual inspection, I found only 143 out of 387 questions after 23.12.31 successfully generated the code (others encountered the issue of endless repeating.)

If we consider only the questions that LLM successfully generates the code, 
the statistic is as follows:
% count_all: 143, count_success: 67
% difficulty_frequency: {'easy': 55, 'medium': 11, 'hard': 1}.

\begin{table}[h!]
\centering
\begin{tabular}{@{}cccccc@{}}
\toprule
\textbf{Setting} &\textbf{Count All} & \textbf{Count Success} & \textbf{Easy} & \textbf{Medium} & \textbf{Hard} \\ \midrule
DeepseekCoder 32B with all solution & 387                & 67                     & 55            & 11              & 1             \\ 

DeepseekCoder 32B with solution generated code &143                & 67                     & 55            & 11              & 1             \\ \bottomrule
\end{tabular}
\caption{LeetCode Questions Summary}
\label{tab:leetcode_summary}
\end{table}

To solve this issue, there are two ways I keep in mind:

1) a grid search on two key hyper-parameters: frequency\_penalty and temperature 

2) write a customized approach that enforces the LLM doesn't use the same tokens when a repeating string is detected

Implement the first approach as it's more simple.

\begin{table}[]
\caption{Performance on LiveCodeBench}
\begin{tabular}{ccccc}
\toprule
              & \multicolumn{4}{l}{Pass@1 on LiveCodeBench} \\ 
          
              & Easy      & Medium     & Hard  & Overall   \\ \midrule    
Qwen2.5       & 0.847     & 0.343      & 0   & 0.398     \\
Tuned Qwen2.5 & 0.815 (\textcolor{green}{3.78\%})    & 0.490 (\textcolor{red}{43.86\%})     & 0   & 0.442 (\textcolor{red}{11.06\%})    \\ 
\bottomrule
\end{tabular}
\end{table}

\subsection{Experiment Plan}
\subsubsection{More LLMs}
Select based on bigcodebench
+ Phi4

++ LiveCodeBench

+ Qwen2.5 14B

\subsection{Baselines}
CodeQwen2.5
COT approaches
QWQ
Skythought
A craft baseline that use the same code but apply QWQ to generate the reasoning steps.


\subsection{More Datasets}
Humaneval and MBPP, where we show our LLM after fine-tuning doesn't have significant difference

EVOPERF or other efficiency benchmark, where we expect our LLM after fine-tuning can be more efficient

Code Contests on function / class level, where we expect our LLM can generate better code



==> sections/background.tex <==


% \textcolor{red}{Can delete the following shits}


% \subsection{SFT Reasoning-Augmented LLM}
% There are several ways to enable LLM perform reasoning-augmented code generation.
% One way is to use reinforcement learning (RL) to train the LLM with reasoning-aware reward functions. However, this approach requires significant amount of compute resources. \textcolor{red}{TODO: number of GPUs for deepseek r1.}
% Alternatively, test-time scaling like chain-of-thought prompting (COT) can enhance LLMs' reasoning capabilities without extensive retraining. COT encourages LLMS to generate reasoning steps before generating code using the inherent reasoning ability of LLMs. While CoT-based approaches have shown improvements in certain tasks, their effectiveness heavily rely on the LLM's inherent reasoning ability, which may not suffice for complex coding problems. Research indicates that CoT's performance gains are limited and depend on highly problem-specific prompts, highlighting its constraints in generalizing to more intricate tasks~\cite{xia2024evaluating}. 
% In this paper, we focus on SFT-based reasoning-augmented LLM, where LLMs are fine-tuned on datasets comprising tuples of coding questions, reasoning steps, and code solutions. During training, the LLM learns to generate reasoning steps followed by the corresponding code solution for a given problem statement. At inference time, the LLM first produces the reasoning steps and then the code solution. This method enables models to learn structured reasoning patterns pertinent to complex coding problems, enhancing their reasoning capabilities without the extensive computational demands associated with RL.





\subsection{Benchmark of Challenging Code Problems}
There are a few famous and commonly-used benchmarks for code generation, e.g., HumanEval~\cite{chen2021humaneval}, MBPP~\cite{austin2021mbpp}, APPS~\cite{hendrycks2021apps}, CodeContests~\cite{li2022codecontests}, and LiveCodeBench~\cite{jain2024livecodebench}.
All of them are packed with test cases to allow execution-based evaluation.
% However, MBPP, released in 2021, consists primarily of beginner-level programming problems that do not necessarily require complex reasoning. APPS and CodeContests offer more challenging problems sourced from competitive programming platforms, but they were released in 2021 and 2022, respectively. 
However, studies have shown that early benchmarks are often included in LLM training data~\cite{jain2024livecodebench}, raising concerns about data contamination.
This issue affects benchmarks such as HumanEval, MBPP, APPS, and CodeContests, all of which are publicly released before 2023.
To avoid the risk of data contamination, this paper focuses on LiveCodeBench, a continuously updated benchmark that aggregates new coding problems from diverse platforms from 2023 to 2025. Since LiveCodeBench allows for the selection of problem subsets based on their release dates, it mitigates data contamination risks and provides a more reliable assessment of LLM performance on unseen, real-world coding challenges across diverse difficulty levels.


% HumanEval includes 164 programming problmes, MBPP includes 1,500 programming problems, APPS includes 10,000 programming problems, CodeContests includes 10,000 programming problems, and LiveCodeBench includes 10,000 programming problems.
% HumanEval includes 164 programming problmes, MBPP includes 1,500 programming problems, APPS includes 10,000 programming problems, CodeContests includes 10,000 programming problems, and LiveCodeBench includes 10,000 programming problems.


% 1. The way to enable reasoning ability of LLM
% There are several ways to enable LLM perform reasoning-augmented code generation.
% One way is to use reinforcement learning (RL) to train the LLM with reasoning-aware reward functions. However, this approach requires significant amount of compute resources. \textcolor{red}{TODO: number of GPUs for deepseek r1.}
% Alternatively, test-time scaling like chain-of-thought prompting (COT) can enhance LLMs' reasoning capabilities without extensive retraining. COT encourages LLMS to generate reasoning steps before generating code using the inherent reasoning ability of LLMs. While CoT-based approaches have shown improvements in certain tasks, their effectiveness heavily rely on the LLM's inherent reasoning ability, which may not suffice for complex coding problems. Research indicates that CoT's performance gains are limited and depend on highly problem-specific prompts, highlighting its constraints in generalizing to more intricate tasks~\cite{xia2024evaluating}. 
% In this paper, we focus on SFT-based reasoning-augmented LLM, where LLMs are fine-tuned on datasets comprising tuples of coding questions, reasoning steps, and code solutions. During training, the LLM learns to generate reasoning steps followed by the corresponding code solution for a given problem statement. At inference time, the LLM first produces the reasoning steps and then the code solution. This method enables models to learn structured reasoning patterns pertinent to complex coding problems, enhancing their reasoning capabilities without the extensive computational demands associated with RL.

% 2. evaluation dataset

% \subsection{Preliminary Study: Can human reasoning benefit LLM code generation?}
% LLMs often struggle with complex coding tasks that require multi-step reasoning and structured problem-solving. To evaluate whether human reasoning can enhance LLM-generated solutions, we conduct a preliminary study examining the impact of incorporating human-validated reasoning steps into code generation.

% This study aims to determine whether explicitly integrating ground-truth reasoning steps improves an LLM’s ability to produce correct and logically consistent code for complex coding problems. Answering this question provides insights into the value of human reasoning and justifies the development of our \dataset.
% One challenge in this preliminary study is the lack of existing datasets that include human-verified reasoning steps for complex coding problems. To address this, we leverage manually curated discussions that share problem-solving insights on competitive programming platforms. These discussions contain problem-solving insights where the discussion format is defaultly organized with intuition (i.e., first thoughts on how to solve this problem), approach (i.e., how to solve this problem), and complexity (i.e., the time and space complexity of the solution). 

% \subsubsection{Experiment Design}
% % \noindent \textbf{Dataset.}
% We randomly select 20 LeetCode problems released from 2024 as the dataset for this preliminary study to prevent the risk of data leakage.
% For each LeetCode problem, we select 10 up-voted discussions from the LeetCode platform which follow the format of intuition, approach, and complexty. We treat those discussions $\mathit{D}$ as approximations of ground-truth human reasoning steps.
% Then for each LeetCode problem $\mathit{P}$, we prodide $\mathit{D}$ at the end of the problem statement and ask the LLM to generate a code solution $\mathit{C}$ that follows $\mathit{D}$ and satisfies $\mathit{P}$.
% We set the other baseline where we ask the LLM to generate the code solution $\mathit{C}$ with self-generated reasoning steps.
% We evaluate the performance of the LLM by checking whether the generated code $\mathit{C}$ passes all the test cases provided by the LeetCode platform.





% . 
% We first conduct 


% Interestingly, we observe that valuable data already exists in the form of natural human reasoning shared on competitive programming and coding contest websites. Platforms such as LeetCode, Codeforces, and Stack Overflow feature rich discussions where developers openly share their thought processes, dissect complex problems, and collaboratively construct robust solutions. These discussions often contain step-by-step reasoning, alternative approaches, and detailed explanations of why certain solutions work while others do not. Such human-validated reasoning is not only comprehensive but also reflects real-world problem-solving strategies that could guide LLMs toward better performance on complex coding tasks.

